Congestion-aware path coordination game with Markov decision process dynamics

Inspired by the path coordination problem arising from robo-taxis, warehouse management, and mixed-vehicle routing problems, we model a group of heterogeneous players responding to stochastic demands as a congestion game under Markov decision process dynamics. Players share a common state-action space but have unique transition dynamics, and each player's unique cost is a {function} of the joint state-action probability distribution. For a class of player cost functions, we formulate the player-specific optimization problem, prove the equivalence between the Nash equilibrium and the solution of a potential minimization problem, and derive dynamic programming approaches to solve the Nash equilibrium. We apply this game to model multi-agent path coordination and introduce congestion-based cost functions that enable players to complete individual tasks while avoiding congestion with their opponents. Finally, we present a learning algorithm for finding the Nash equilibrium that has linear complexity in the number of players. We demonstrate our game model on a multi-robot warehouse \change{path coordination problem}, in which robots autonomously retrieve and deliver packages while avoiding congested paths.

==> acknowledgments.tex <==
\section{Acknowledgments}
We would like to thank De Meng, Maryam Fazel and Mehran Mesbahi for their help.

==> individualPlayer.tex <==
\section{Individual Players}

To analyze how the penalty functions affect the individual player's decision making, we develop their perspective through the value function formulation, make connections to Q-Functions, and show that the penalties directly affect the value functions of individual players.

\subsection{Dual Formulation: Value Iteration}
It is well know that the dual of the linear programming MDP optimization problem is the dynamic programming formulation of the same problem. Here we show that in the non-linear, state dependent case, the dual constraints forms the dynamic programming problem new players joining the game would solve at time $t$.

Individual players try to optimize their value functions through solving the dual of the primal MDP problem. Given the MDP game primal problem, Eqn. \ref{MDP game}, the dual can be written as:  
\begin{equation}
\begin{aligned}
\max_{V_{ts}}  & \quad \sum_s V_{0s}p_s \\
\text{s.t } & V_{ts} \leq \sum_{s'} P(s'| s, a)V_{t+1,s'} + \ell_{tsa}(y_{tsa}) \quad \\
& \forall \, s \in \mc{S}, a\in \mc{A}, t \in [T-1] \\
& V_{Ts} \leq \ell_{tsa}(y_{tsa}) \quad \forall \, s \in \mc{S},\,\, a\in \mc{A}
\end{aligned} \label{unconstrained dual}
\end{equation}
From this we can derive the value iteration method shown for latency functions $\ell_{tsa}(y_{tsa}) $. Let the Q function be defined as following: 
\begin{equation}\label{q function}
Q_{tsa}(y_{tsa}) = \sum_{s'} P(s'| s, a)V_{t+1,s'} + \ell_{tsa}(y_{tsa}) \\
\end{equation}
The difference $V^*_{ts} -  Q_{tsa}(y^*_{tsa}) = \mu^*_{tsa} \geq 0$ is the dual variable of constraint $y_{tsa} \geq 0 $, and is also the inefficiency of the action $a$. Any action $\bar{a} $ whose inefficiency is zero is the optimal action at that particular state and time. 


Which leads to the value iteration method Alg. \ref{value iteration}. 
\begin{algorithm}
\caption{Value iteration}
\begin{algorithmic}[h]
\Require \(R\), \(P\).
\Ensure \(V^\star\), \(\pi^\star\).
\ForEach{\(s,\in\mathcal{S}\)}
\State{\(V^\star_{Ts}= \underset{a\in\mathcal{A}}{\mbox{min}} \,\,\ell_{Tsa}(y_{Tsa})\)}
\State{\(\pi^\star_{Ts}= \underset{a\in\mathcal{A}}{\argmin} \,\,\ell_{Tsa}(y_{Tsa})\)}
\EndFor
\For{\(t=T-1, T-2, \ldots, 0\)}
\ForEach{\(s\in\mathcal{S}\)}
\State{\(\displaystyle V^\star_{ts}= \underset{a\in\mathcal{A}}{\mbox{min}}\,\, Q_{tsa}(y_{tsa})\)}
\State{\(\displaystyle \pi^\star_{ts} = \underset{a\in\mathcal{A}}{\argmin}\,\, Q_{tsa}(y_{tsa})\)}
\EndFor
\EndFor
\end{algorithmic}
\label{value iteration}
\end{algorithm}

\begin{theorem}
Assuming existing players have reached nash equilibirum, and the rewards are state dependent $R_{tsa}(y_{tsa}) $, algorithm \ref{value iteration} with optimal  $y^*_{tsa} $ is the dynamic programming problem that any new player solves entering the game at time $t $.

Furthermore, the best reward that the new player can gain is defined by 
\[\min_s V^*_{ts}\]
\end{theorem}

\begin{proof}
Since the algorithm depends on current state-action distribution, $y_{tsa}$. At Nash Equilibrium the constraints would be: 
\[V_{ts} \leq \sum_{s'} P(s'| s, a)V_{t+1,s'} + \ell_{tsa}(y^*_{tsa}) \]
\[V_{Ts} \leq \ell_{tsa}(y^*_{tsa}) \]
Any player entering at time t would need to maximize its value function according to $V_{ts} $. Since the game is non-atomic, the new player would not affect the state depedent reward functions. Therefore, the new player's optimal policy can be found from algorithm \ref{value iteration}.
 % optimal policy for each individual player will be different in the finite horizon case.  
\end{proof}



Suppose we impose constraint $y_{t\bar{s}\bar{a}} \leq d_{t\bar{s}\bar{a}} $ for one state $\bar{s} $ and all times t, and suppose it was violated during time step $\bar{t}$. From an individual game player's perspective, the exact penalty function coefficients $k_t(\bar{s},\bar{a}) $,  directly offsets the value functions at constrained optimal $y_c^*(s,a)$.  

Using the exact penalty theorem, we find the minimum coefficient $k_{\bar{t}\bar{s}\bar{a}} \geq \tau^*_{\bar{t}\bar{s}\bar{a}} $ to ensure that the optimal solutions are between the penalized problem and the unconstrained problem are the same. However in order to ensure that the next player will also avoid the constraints, additional "toll" need to be charged. 


\begin{theorem}
In addition to $\tau^*_{\bar{t}\bar{s}}$ the dual variable's optimal value corresponding to the constraint $y_{t\bar{s}\bar{a}} \leq d_{t\bar{s}} $ in problem \eqref{MDP game}. Let 
\[k_{\bar{t}\bar{s}\bar{a}} > \max\{\tau^*_{\bar{t}\bar{s}\bar{a}}, \mu_{\bar{t}\bar{s}a_{new}}   \}\]
\[a_{new} = \text{argmin}_{a \neq \bar{a}} Q_{\bar{t}\bar{s}a} \]
Then we can guarantee that the next player will not choose to violate the constraint $y_{\bar{t}\bar{s}\bar{a}} \leq d_{\bar{t}\bar{s}\bar{a}} $

\end{theorem}

\begin{proof}
From the exact penalty theorem, the solution to the unconstrained problem \eqref{MDP Game} and the constrained problem \eqref{cMDP game} share the same value and argument. 
\begin{equation}
\begin{aligned}
\underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \sum\limits_{a\in\mathcal{A}} \int_0^{y_{tsa}}\ell_{tsa}(x)dx\\
\mbox{s.t.} &\sum\limits_{a\in\mathcal{A}} y_{t+1, sa} = \sum\limits_{s'\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}P_{s'as}y_{ts'a}, \quad t\in[T-1],\\
&\sum\limits_{a\in\mathcal{A}}y_{0sa}=p_s,\\
& y_{t\bar{s}\bar{a}} \leq d_{t\bar{s}\bar{a}}, \\
&y_{tsa}\geq 0,\quad \forall s\in\mathcal{S}, a\in\mathcal{A}, t\in[T]
\end{aligned}\label{cMDP game}
\end{equation}

For at the optimal solution of this constrained MDP game, the dual value iteration method occurs according to algorithm \ref{constrained value iteration}. Here we see the value of $k_{t\bar{s}\bar{a}} $ directly offsets the Q-functions at the times when the unconstrained solution violated the state constraints.

\begin{algorithm}
\caption{Constrained Value iteration at constrained optimal $y_c^* $}
\begin{algorithmic}[h]
\Require \(R\), \(P\).
\Ensure \(V^\star\), \(\pi^\star\).
\ForEach{\(s,\in\mathcal{S}\)}
\State{\(
V^\star_{Ts}= \underset{a\in\mathcal{A}}{\mbox{min}} \,\,Q_{Tsa} + k_T(s,a)\)}
\State{\(
\pi^\star_{T}(s)= \underset{a\in\mathcal{A}}{\argmin} \,\,Q_{Tsa} + k_T(s,a)\)}
\EndFor
\For{\(t=T-1, T-2, \ldots, 0\)}
\ForEach{\(s\in\mathcal{S}\)}
\State{\(\displaystyle V^\star_{t}(s)= \underset{a\in\mathcal{A}}{\mbox{min}}\,\, Q_{tsa} + k_t(s,a)\)}
\State{\(\displaystyle \pi^\star_{t}(s) = \underset{a\in\mathcal{A}}{\argmin}\,\, Q_{tsa}+ k_t(s,a)\)}
\EndFor
\EndFor
\end{algorithmic}
\label{constrained value iteration}
\end{algorithm}

Suppose the violated constraint occurs at $\bar{t}, \bar{s}, \bar{a} $. Let $\tilde{\mu} $ be the smallest inefficiency of the set of actions available at $\bar{s} $, excluding optimal action $\bar{a} $. If $k_{\bar{t}\bar{s}\bar{a}} > \tilde{\mu} $, then $\bar{a} $ is no longer the optimal, and so the player will not choose $\bar{a} $ as optimal policy. Therefore, the original constraint $y_{t\bar{s}\bar{a}} \leq d_{t\bar{s}\bar{a}} $ cannot be violated at $\bar{t} $ if the original solution was feasible. 

Since $k_{\bar{t}\bar{s}\bar{a}} > \tau^*_{\bar{t}\bar{s}\bar{a}} $, then we still satisfy the exact penalty theorem, and so the optimal solution and arguments of the penalized problem still correspond to the constrained problem's solution and arguments. 
\end{proof}

\begin{theorem}
For a new player entering the game at time $t $, their best expected reward is upperbounded by the optimal value function at time $t $. 
\[\max_{s} \tilde{V}_{ts} \]
Where $\tilde{V}_{ts} $ is the result of solving algorithm \ref{constrained value iteration}. Furthermore, the player can achieve this value by starting at state $s = \text{argmax} V_{ts} $ and follow optimal policy $\pi_{ts}^* $from algorithm \ref{constrained value iteration}.
\end{theorem}
\begin{proof}
This follows from the fact that the value functions is equivalent to the expected sum of rewards over time.
\end{proof}
% \begin{proof}
% 
% Note that the KKT conditions of the primal optimization problem with the exact penalty terms gives the same value iterations as the not penalized, unconstrained problem when the constraints are not active. But gives the following inequalities when the constraints are active. 
% \[ \tilde{V}_t(s) \leq \sum_{s'} P(s'| s, a)\tilde{V}_{t+1}(s') + R_t(s,a) + k_t(s,a) \quad \forall \, s \in \mc{S}, a\in \mc{A}, t \in [T-1] \]
% \[ \tilde{V}_T(s) \leq R_T(s,a)+ k_T(s,a) \quad \forall \, s \in \mc{S},\,\, a\in \mc{A} \]

% Then since $k_t(s,a) > \tau_t^*(s,a) $, we note that where $\tau_t^*(s,a) = 0 $, we can remove the constraint and equivalently set $k_t(s,a) = 0 $. Therefore, the previous KKT conditions hold both when constraints are active and not active. Finally they lead to the value iteration method outlined in Algorithm \ref{constrained value iteration}.

% Finally for any additional player with a choice of starting position, their optimal choice to minimize $\tilde{V}_0$ would be to choose the state with the smallest initial value function. 
% \end{proof}

% \begin{theorem}
% Assume there exists a feasible, non-zero toll, $\tau^* $ corresponding to constraint  $y_t(s,a) \leq d_t(s,a)$ for Eqn. \ref{MDP}. Then for $V_0^*(s)$ the optimal solution of the dual problem,
% % For the following MDP problem, with the added constraint  $y_t(s,a) \leq d_t(s) $. 
% % \begin{equation}\label{MDP}
% % \begin{aligned}
% % \text{maximize}\quad &\sum_{t\in\mathcal{T}} \sum_{s\in\mathcal{S}} \sum_{a\in\mathcal{A}} \int_0^{y_t(s,a)} c_t(s,a) \partial y_t(s,a) \\
% % \text{s.t.} \,\,& \sum\limits_{a\in\mathcal{A}} y_{t+1}(s', a) = \sum\limits_{s\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}\Gamma(s'\mid s, a)y_t(s, a),\\
% % &\sum\limits_{a\in\mathcal{A}}y_0(s, a)=p_0(s),\\
% % &y_t(s, a)\geq 0,\\
% % \end{aligned}
% % \end{equation}
% then any additional agents added to network will avoid the constrained state. 
% \end{theorem}
% \begin{proof}
% Consider an optimal solution to the unconstrained problem, Eqn. \ref{MDP}, $y^*_t(s,a)$, for some convex cost function $R_t(s,a)$. 
% \begin{equation}
% \begin{aligned}
% \underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \sum\limits_{a\in\mathcal{A}} R_t(s,a)\\
% \mbox{s.t.} &\sum\limits_{a\in\mathcal{A}} y_{t+1}(s,a) = \sum\limits_{s'\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}P(s'|s,a)y_{t+1}(s,a), \quad t\in[T-1],\\
% &\sum\limits_{a\in\mathcal{A}}y_0(s,a)=p(s),\\
% &y_t(s,a)\geq 0,\quad \forall s\in\mathcal{S}, a\in\mathcal{A}, t\in[T]
% \end{aligned}\label{MDP}
% \end{equation}
% Suppose constraints $y_t(\bar{s},\bar{a}) \leq d_t$ are added for all t. Let $x_t^*(s,a)$ be the solution to Eqn.\ref{cMDP}. 
% \begin{equation}
% \begin{aligned}
% \underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \sum\limits_{a\in\mathcal{A}} R_t(s,a)\\
% \mbox{s.t.} &\sum\limits_{a\in\mathcal{A}} y_{t+1}(s,a) = \sum\limits_{s'\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}P(s'|s,a)y_{t+1}(s,a), \quad t\in[T-1],\\
% &\sum\limits_{a\in\mathcal{A}}y_0(s,a)=p(s),\\
% &y_t(s,a)\geq 0,\quad \forall s\in\mathcal{S}, a\in\mathcal{A}, t\in[T] \\
% &y_t(\bar{s},\bar{a}) \leq d_t, \quad \forall  t\in[T]
% \end{aligned}\label{cMDP}
% \end{equation}
% Finally consider the exact penalty from Eqn. \ref{cMDP}, in the form : $\sum_{t\in[T]} k_t(y_t(\bar{s},\bar{a}) - d_t)_+ $, where $k_t > \tau^*_t $, the optimal dual variables, and the optimal solution of the unconstrained problem, Eqn.\ref{exMDP}, with the exact penalty term, $z^*_t(s,a) $. 
% \begin{equation}
% \begin{aligned}
% \underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \sum\limits_{a\in\mathcal{A}} R_t(s,a) + \sum_{t\in[T]} k_t(y_t(\bar{s},\bar{a}) - d_t)_+\\
% \mbox{s.t.} &\sum\limits_{a\in\mathcal{A}} y_{t+1}(s,a) = \sum\limits_{s'\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}P(s'|s,a)y_{t+1}(s,a), \quad t\in[T-1],\\
% &\sum\limits_{a\in\mathcal{A}}y_0(s,a)=p(s),\\
% &y_t(s,a)\geq 0,\quad \forall s\in\mathcal{S}, a\in\mathcal{A}, t\in[T] \\
% \end{aligned}\label{exMDP}
% \end{equation}

% If $y^*_t(\bar{s},\bar{a}) < d_t $, then adding additional population $\partial y $ will not violate the constraints either. Therefore we only consider the case when the constraint is active. Ie. $y^*_t(\bar{s},\bar{a}) \geq d_t $.


% The gradient of the Lagrangian with respect to $y_t(s,a) $ gives rise to value iteration. For each $t = 0\cdots, T-1 $, the gradient of the constrained Lagrangian of Eqn.\ref{cMDP} with respect to $y_t(\bar{s}, \bar{a}) $ is the following.

% \[ \nabla R_t(\bar{s}, \bar{a})  + \sum_{s'} P(s'| \bar{s}, \bar{a})  + \mu_t(\bar{s}, \bar{a}) - V_t(\bar{s}) + \tau_t \]

% For optimal $x_t^*(\bar{s},\bar{a}), V^*_t(\bar{s}), V^*_{t+1}(\bar{s}), \mu^*_t(\bar{s}, \bar{a}) $, $\frac{\partial L_c}{y_t(\bar{s}, \bar{a})} = 0 $. Since we assumed that the constraint is active, $ x_t^*(\bar{s},\bar{a})  = d_t > 0 $. From complimentary slackness, $\mu^*_t(\bar{s},\bar{a}) = 0 $. 

% \[ \nabla R_t(\bar{s}, \bar{a})  + \sum_{s'} P(s'| \bar{s}, \bar{a})V_{t+1}(s') - V_t(\bar{s}) + \tau_t = 0\]

% Similarly for a different action $a_2 $,  the following is true at optimal values, $x_t^*(\bar{s},a_2), V^*_t(\bar{s}), V^*_{t+1}(\bar{s}), \mu^*_t(\bar{s}, a_2) $, $\frac{\partial L_c}{y_t(\bar{s}, a_2)} = 0  $

% \[ \nabla R_t(\bar{s}, a_2)  + \sum_{s'} P(s'| \bar{s}, a_2)V_{t+1}(s')  + \mu_t(\bar{s}, a_2) - V_t(\bar{s}) = 0\]

% The two KKT conditions have $V_t(\bar{s}) $ and $V_{t+1}(s') \quad \forall s' \in \mathcal{S}$ in common, solving for $\tau_t $:
% \begin{equation}
% \begin{split}
% \tau_t & = \nabla R_t(\bar{s}, a_2) - \nabla R_t(\bar{s}, \bar{a}) \\
% & + \sum_{s'} P(s'| \bar{s}, a_2)V_{t+1}(s')  - \sum_{s'} P(s'| \bar{s}, \bar{a})V_{t+1}(s') \\
% & + \mu_t(\bar{s}, a_2) \\
% \end{split}
% \end{equation}

% From exact penalty theorem, Eqn.\ref{exMDP} must have the same solution arguments as Eqn.\ref{cMDP}. Let $W_t(\bar{s}) $ be the value functions for the dual of Eqn.\ref{exMDP}. The following relationship must hold: 
% \begin{equation}
% \begin{aligned}
% \nabla R_t(\bar{s}, \bar{a})  + \sum_{s'} P(s'| \bar{s}, \bar{a})W_{t+1}(s')) - V_t(\bar{s})  &= \\
% \nabla R_t(\bar{s}, a_2)  + \sum_{s'} P(s'| \bar{s}, \bar{a})W_{t+1}(s')) - V_t(\bar{s})  &
% \end{aligned}
% \end{equation}


% If $y^*_t(\bar{s},\bar{a}) > d_t$, and $x^*_t(\bar{s},\bar{a}) < d_t$, then additional player $\partial y $ will also not violate the constraints. 

% However if $y^*_t(\bar{s},\bar{a}) > d_t$, and $x^*_t(\bar{s},\bar{a}) = d_t$, then it can be shown that the additional player $\partial y $ will definitely not choose action $\bar{a} $. From KKT conditions, $\tau^*_t$ is non-zero where $y_t^*(\bar{s},\bar{a}) > d_t $. 

% Suppose for $t_c$, $y^*_{t_c}(\bar{s},\bar{a}) $ lies outside the constrained domain, then since problem is linear, the optimal constrained solution must lie on the boundary of the constraint, $x_{t_c}^*(\bar{s},\bar{a})  = d(\bar{s},\bar{a})  $. 


% At $t_c$, the value functions to the dual of Eqn. \ref{exMDP} is
% \[
% V_{t_c}(s_c)  = \max_a f(a) = c_{t_c}(s_c, a) + \sum_{s'}\Gamma (s' | s_c, a)V_{t_c + 1}(s')
% \]
% The policy is 
% \[
% \pi_{t_c}(s_c)  = \argmax_a c_{t_c}(s_c, a) + \sum_{s'}\Gamma (s' | s_c, a)V_{t_c + 1}(s')
% \]
% If $ y_{t_c}^*(s_c,a_c) > d_{t_c}(s_c,a_c) $ and $x_{t_c}^*(s_c,a_c) = d_{t_c}(s_c,a_c) $, then there exists alternative $a' $ such that $f(a') > f(a_c) $. Therefore any additional agent will not choose $a_c $, instead will choose $a' $, and therefore avoid the constrained state action pair. 
% \end{proof}

==> method2.tex <==
\section{Unknown Initial Distribution}

(I believe this is the the most general way to constrain the policy to maintain safety in the MDP.)

I think we want to solve the following problem for all $t' = 0,\dots,T$.

\begin{align}
\max_{y,p_{t'}} & \quad \sum_{s} \sum_{a} \Gamma_{t'}(s'|s,a) K_{t'}(s,a)p_{t'}(s) \\
\text{s.t.} & \quad \sum_s \sum_a y_0(s,a) = 1 \notag \\
& \quad \sum_a y_{t+1}(s',a) = \sum_{s \in \mathcal{S}} \sum_{a \in \mathcal{A}} \Gamma_t(s'|s,a) y_t(s,a) \notag \\
& \qquad \qquad \qquad \qquad \qquad \qquad t = 0,\dots,t'-1  \notag \\
& \quad \sum_a y_{t'}(s,a) = p_{t'}(s) \notag \\
& \quad 0 \leq y_t(s,a) \leq d_t(s,a) \qquad t=0,\dots,t' \notag
\end{align}

We want to get a bound for the maximum amount of mass in state $s^*$.  
\begin{align}
\min & \quad \lambda + \sum_t\sum_s\sum_a d_t(s,a)\tau_t(s,a) \\
\text{s.t.} & \quad \lambda = V_0(s)+\tau_0(s,a) \qquad \qquad \qquad \forall s \in \mathcal{S} \notag \\
& \quad V_t(s') = \sum_s \Gamma_t(s'|s,a)\Big(V_{t+1}(s)+\mu_t(s,a)\Big)+\tau_t(s,a) \notag \\
& \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \forall a \in \mathcal{A} \notag \\
& \quad V_{t'} = \sum_a \Gamma_{t'}(s^*|s,a)K_{t'}(s,a) + \tau_{t'}(s,a) \notag
\end{align}


\section{Useless Stuff}

We now consider the case where the initial distribution is not known a-priori but rather only constrained to be within some set.  We assume $p_0 \in \mathcal{P}_0$.  We first consider box capacity constraints on $p_0 \leq d_0$ and defining the least conservative constant constraints on the policy that keep the set invariant.  Set $\bar{d}_0 = d_0$. Let $\bar{d}_t$ be upper bounds on the state distribution at time $t$.  We now derive bounds on the entries of $K_t(s,a)$.  If the constraint at the next time step 
\begin{align}
d_{t+1}(s')= \Gamma_t(s'|s,a)K_t(s,a)\bar{d}_t(s)
\end{align}
\begin{align}
K_t(s,a) = 
\frac{d_{t+1}(s')}{\Gamma_t(s'|s,a)\bar{d}_t(s)}
\end{align}
\begin{align}
D_t(s,a) = \min \left\{\min_{s'}
\frac{d_{t+1}(s')}{\Gamma_t(s'|s,a)\bar{d}_t(s)},1
\right\}
\end{align}
\begin{align}
\bar{d}_{t+1}(s') = \max_{y_t} & \quad \sum_s \sum_a \Gamma_t(s'|s,a)y_t(s,a) \\ 
\text{s.t.}& \quad \sum_a y_t(s,a) \leq \bar{d}_t(s) \notag \\
& \quad \sum_{s,a} y_t(s,a) = 1 \notag \\
& \quad y_t(s,a) \leq \text{diag}(y_t\mathbf{1})D_t(s,a) \notag
\end{align}

==> population.tex <==
\subsection{Population Perspective: Numerical Method}\label{sec:dualFormulation}

After the social planner has offered incentives, the population plays the Wardrop equilibrium defined by modified rewards~\eqref{eq:generalReward}; this equilibrium can be computed using the Frank Wolfe (FW) method~\cite{freund2016new}, given in Algorithm~\ref{alg:MSA}, with known optimal variables $\{\tau_i^{\star}\}$. 

FW is a numerical method for convex optimization problems with continuously differentiable objectives and compact feasible sets \cite{powell1982convergence}, including routing games.   One advantage of this learning paradigm is that the population does not need to know the function $r(\cdot)$. Instead, they simply react to the realized rewards of previous game at each iteration. It also provides an interpretation for how a Wardrop equilibrium might be asymptotically reached by agents in MDPCG in an online fashion.

Assume that we have a repeated game play, where players execute a fixed strategy determined at the start of each game. At the end of each game $k$, rewards of game $k$ based on $y^k_{tsa}$ are revealed to all players. FW models the population as having two sub-types: \emph{adventurous} and \emph{conservative}. Upon receiving reward information $\ell_{tsa}(y^{k}_{tsa})$, the adventurous population decides to change its strategy while the conservative population does not. To determine its new strategy, the adventurous population uses value iteration on the latest reward information---i.e.~Algorithm \ref{alg:valueIteration}---to compute a new optimal policy. Their resultant density trajectory is then computed using Algorithm \ref{alg:policy iteration}. The step size at each iteration is equivalent to the fraction of total population who switches strategy.  
The stopping criteria for the FW algorithm is determined by the Wardrop equilibrium notion---that is, as the population iteratively gets closer to an optimal strategy, the marginal increase in potential decreases to zero.
%; equivalently, no individual can gain any further advantage by switching strategies. 
\begin{algorithm}
\caption{Value Iteration Method}
\begin{algorithmic}[h]
\Require \(r\), \(P\).
\Ensure \( \{\pi^{\star}_{ts}\}_{ t \in [T], \, s\in \mc{S}} \)
\For{\(t=T, \ldots, 1\)}
% 	\ForEach{\(s\in\mathcal{S}\)}
		\State{\(\displaystyle V_{ts}= \underset{a\in\mathcal{A}}{\mbox{max}}\, Q_{tsa}\), \(\displaystyle \pi^{\star}_{ts} = \underset{a\in\mathcal{A}}{\mbox{argmax}}\, Q_{tsa},\ \forall \ s \in \mc{S}\)} \Comment{Eqn.~\eqref{eq:qvalue}}
% 		\State{\(\qquad \)}
% 		\State{\(\displaystyle \pi^{\star}_{ts} = \underset{a\in\mathcal{A}}{\mbox{argmax}}\,\, Q_{tsa}\)}  \Comment{Eqn.~\eqref{eq:qvalue}}
% 	\EndFor %\ForEach{\(s\in\mathcal{S}\)}
\EndFor %\For{\(t=T-1, T-2, \ldots, 0\)}
\end{algorithmic}
\label{alg:valueIteration}
\end{algorithm}
\begin{algorithm}
\caption{Retrieving density trajectory from a policy }
\begin{algorithmic}[h]
\Require \(P\), \(p\), \(\pi\).
\Ensure \(\{d_{tsa}\}_{t \in[T], s\in\mc{S}, a\in\mc{A}}\)
\State{\(d_{tsa} = 0, \ \forall \ t \in [T], s \in \mc{S}, a \in \mc{A}\)}
\State{\(d_{1s\pi_{1s}} = p_s, \ \forall s \in \mc{S}\)}
\For{\(t=2, \ldots, T\)}
% 	\ForEach{\(s\in\mathcal{S}\)}
	   % \If{\(t = 1\)}
	   %     \State{\(d_{1s\pi_{1s}} = p_s\)}
	   % \Else
		    \State{\(d_{ts(\pi_{ts})} = \sum\limits_{a \in \mc{A}}\sum\limits_{s' \in \mc{S}} P_{t-1,ss'a}d_{t-1,s'a}, \ \forall\ s \in \mc{S} \)}
% 		\EndIf
% 	\EndFor % \ForEach{\(s\in\mathcal{S}\)}
\EndFor % \For{\(t=T-1, T-2, \ldots, 0\)}
\end{algorithmic}
\label{alg:policy iteration}
\end{algorithm}
\begin{algorithm}
\caption{Frank Wolfe Method with Value Iteration}
\begin{algorithmic}[h]
\Require \(\bar{\ell}\), \(P\), \(p_s\), \(N\), \(\epsilon\).
\Ensure \(\{y^{\star}_{tsa}\}_{t \in [T], s\in\mc{S}, a \in \mc{A}}\).
\State{\( y^0 = 0 \in \reals^{T \times|\mc{S}| \times |\mc{A}|} \)}
\For{\(k = 1, 2, \ldots, N\)}
    \State{\(c^k_{tsa} = \bar{\ell}_{tsa}(y^k)\), \(\quad \forall \,\, t \in [T], s \in \mc{S}, a \in \mc{A}\)}
	\State{\(\pi_{ts} = \) \Call{ValueIteration}{\(c^k\), \(P\)}}
	\Comment{Alg.~\ref{alg:valueIteration}}
	\State{\(d^k\) = \Call{RetrieveDensity}{\(P, p_s, \pi_{ts}\)}}\Comment{Alg.~\ref{alg:policy iteration}}
	%Algorithm~\ref{alg:policy iteration} 
% 	\State{\( \alpha^k =  \)}
	\State{\( y^k = (1 -  \frac{2}{k+1})y^{k-1} +  \frac{2}{k+1} d^k\)}
	\State{Stop if }
	\State{\(\quad \sum\limits_{t\in[T]} \sum\limits_{s\in\mc{S}} \sum\limits_{a\in\mc{A}}\Big(c^k_{tsa} - c^{k-1}_{tsa}\Big)^2 \leq \epsilon\)}
\EndFor
\end{algorithmic}
\label{alg:MSA}
\end{algorithm}

In contrast to implementations of FW in routing game literature, Algorithm \ref{alg:MSA}'s descent direction is determined by solving an MDP \cite[Section~4.5]{puterman2014markov} as opposed to a shortest path problem from origin to destination \cite[Sec.4.1.3]{patriksson2015traffic}. %In MDPCG's, solving the shortest path problem is replaced by solving an MDP.
%A notable departure from routing games is the replacement of shortest path problem from origin to destination by dynamic programming in Algorithm \ref{alg:valueIteration}.  
Algorithm~\ref{alg:MSA} is guaranteed to converge to a Wardrop equilibirum if the predetermined step sizes decrease to zero as a harmonic series \cite{freund2016new}---e.g., $\frac{2}{k+1}$.
%; examples of other such step size sequences can be found in \cite{powell1982convergence}. 
FW with predetermined step sizes has been shown to have sub-linear worst case convergence in routing games \cite{powell1982convergence}. 
%Therefore, a predetermined scheme is far from optimal for convergence to a Wardrop equilibrium. 
On the other hand, replacing fixed step sizes with optimal step sizes found by a line search method leads to a much better convergence rate.
 




% It can be adapted to the stochastic nature of MDPCG by treating subproblems as MDPs with state-independent reward functions, and solving them with a value iteration method that returns deterministic policies. Frank Wolfe with value iteration is outlined in Algorithm \ref{MSA}. 



%the population we present a fixed step size Frank Wolfe (FW) method for solving \eqref{CMDPCG} with known optimal variables 
 
% In addition to solving \eqref{CMDPCG}, FW 
% In addition to solving \eqref{CMDPCG}, FW verifies the \emph{Fictitious Play} property of MDPCG as a potential game, where the iterative solution of FW provides a valid finite improvement path (FIP) \cite{monderer1996potential}. 
%The algorithm is outline in~\ref{MSA}.  

%Consider the modified reward function, \eqref{eq:generalReward}, and penalty functions $\tau_i \frac{\partial g_i}{\partial y_{tsa}}(y)$.
% In the dual formulation of \eqref{mdp game}, equiva 
% The dual of \eqref{mdp game} can be derived with game players' individual value function as the optimization variable \cite{MDPCongestionGame}. Equivalently, solving the dual formulation is the goal of individual players. In the constrained case, the same idea applies to a more generalized objective, which is equivalent to taking Lagrangian of \eqref{constrained lagrangian} as the optimization objective:
% \begin{equation}
% \max_{y_{tsa}} L(y_{tsa}, \mu_{tsa}, V_{tsa},\tau_{t\bar{s}}, \sigma_{t\bar{s}})
% \label{unconstrained lagrangian}
% \end{equation}
% Note that Eqn.\eqref{unconstrained lagrangian} is now unconstrained in state densities $y_{tsa} $., therefore the unconstrained dual formulation is: 
% \begin{equation}
% \begin{aligned}
% \underset{V_{ts}, c_{tsa}}{\mbox{min.}} & \sum\limits_{s \in \mc{S}} V_{0s}p_s - \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \sum\limits_{a\in\mathcal{A}} \int_{\ell_{tsa}(0)}^{c_{tsa}}\ell_{tsa}^{-1}(x)dx\\
% \mbox{s.t.} & V_{Ts} \geq c_{Tsa} - \tau_{Ts} + \sigma_{Ts}, \\
% &V_{ts} \geq c_{tsa} + \sum_{s'} P_{ts'ssa}V_{t+1,s'} - \tau_{ts} + \sigma_{ts},\\
% & \quad \quad \forall a \in \mc{A}, s \in \mc{S}\\
% \end{aligned}\label{dual CMDPCG}
% \end{equation}
% This formulation models the perspective of individual players. The optimization variable, $V_{ts} $, is the value of the generalized objective that players are trying to maximize, and $c_{tsa} $ is the final marginal state-action objective value that the players gain. 

%The penalties can be seen as tolls/rewards on the original reward function, to encourage the game population to achieve constraints $g_i$. When the dual variables $\tau_i$ are optimal, $\bar{\ell}_{tsa} $ represents the modified reward function that can be optimized to achieve Wardrop Equilibrium. 







% \subsection{State Dependent Rewards}
% From \cite{MDPCongestionGame}, the dual of the MDP-CG primal formulation \eqref{mdp game} is equivalent to the recursively maximized value functions that individual players solve. Here we show that in the constrained case, the penalty functions introduce a toll to the value functions.

% In \cite{MDPCongestionGame}, it was proved that the dual of the unconstrained MDP-CG game is equivalent to an incremental value iteration method outlined in Algorithm. \eqref{value iteration}.
% \begin{algorithm}
% \caption{Value Iteration}
% \begin{algorithmic}[h]
% \Require \(\ell_{tsa}\), \(P_{ts'sa}\), \(p_s\), \(N\).
% \Ensure \(V^\star\), \(\pi^\star\).
% \State{\( \alpha =  1/N \)}
% \State{\( y_0 = 0 \in \reals^{|\mc{S}| \times |\mc{A}|} \)}
% % \ForEach{\( s \in \mc{S}, a\in \mc{A}, t \in\)}
% % \EndFor
% % \State{\(\)}
% \For{\(k =  1, 2, \ldots, N\)}
% \ForEach{\(s,\in\mathcal{S}\)}
% \State{\(V^\star_{Ts}= \underset{a\in\mathcal{A}}{\mbox{min}} \,\,\ell_{Tsa}(y_{k-1})\)}
% \State{\(\pi^\star_{Ts}= \underset{a\in\mathcal{A}}{\argmin} \,\,\ell_{Tsa}(y_{k-1})\)}
% \EndFor
% \For{\(t=T-1, T-2, \ldots, 0\)}
% \ForEach{\(s\in\mathcal{S}\)}
% \State{\(\displaystyle V^\star_{ts}= \underset{a\in\mathcal{A}}{\mbox{max}}\,\, \ell_{tsa}(y_{k-1})\)}
% \State{\(\displaystyle \pi^\star_{ts} = \underset{a\in\mathcal{A}}{\argmax}\,\, \ell_{tsa}(y_{k-1})\)}
% \EndFor %\ForEach{\(s\in\mathcal{S}\)}
% \EndFor %\For{\(t=T-1, T-2, \ldots, 0\)}
% \EndFor
% \end{algorithmic}
% \label{value iteration}
% \end{algorithm}

% \begin{algorithm}
% \caption{Policy Iteration}
% \begin{algorithmic}[h]
% \Require \(\ell_{tsa}\), \(P_{ts'sa}\), \(p_s\), \(\pi_{ts}\).
% \Ensure \(x_{ts}\), \(y_{tsa}\).
% \State{\(x = 0 \in \reals^{|\mc{S}| \times |\mc{A}|} \)}
% \State{\(x = 0 \in \reals^{|\mc{S}| \times |\mc{A}|} \)}
% \ForEach{\(s\in\mathcal{S}\)}
% \State{\(x_{0s\pi^*_{0s}} = p_s\)}
% \EndFor % \ForEach{\(s\in\mathcal{S}\)}
% \For{\(t=0, 1, \ldots, T-1\)}
% \ForEach{\(s\in\mathcal{S}\)}
% \State{\(y^{int}_{ts\pi^*_{ts}} = \)}
% \EndFor % \ForEach{\(s\in\mathcal{S}\)}
% \EndFor % \For{\(t=T-1, T-2, \ldots, 0\)}
% \end{algorithmic}
% \label{value iteration}
% \end{algorithm}
% % Consider the following primal problem with a state dependent, non-linear reward function $\ell_{tsa}(y_{tsa}) $:
% % \begin{equation}
% % \begin{aligned}
% % \underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \sum\limits_{a\in\mathcal{A}} \int_0^{y_{tsa}}\ell_{tsa}(x)dx\\
% % \mbox{s.t.} &\sum\limits_{a\in\mathcal{A}} y_{t+1, sa} = \sum\limits_{s'\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}P_{sas'}y_{ts'a}, \quad t\in[T-1],\\
% % &\sum\limits_{a\in\mathcal{A}}y_{0sa}=p_s,\\
% % &y_{tsa}\geq 0,\quad \forall s\in\mathcal{S}, a\in\mathcal{A}, t\in[T]
% % \end{aligned}\label{mdp game}
% % \end{equation}


% % From the positivity constraint on $\mu_{tsa} $, and complimentarity condition of terms $\mu_{tsa}y_{tsa}$, the KKT conditions can be written as: 
% % \begin{equation}
% % \begin{aligned}
% % t = 0: & \sum\limits_{a\in\mathcal{A}}y_{0sa}=p_{0s}\\
% % t = 0 \cdots T-1: & V_{ts} = \min_a \ell_{tsa}(y_{tsa}) + \sum_{s'}P_{s'sa}V_{t+1,s'} \\
% % & \sum\limits_{a\in\mathcal{A}} y_{t+1, sa} = \sum\limits_{s'\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}P_{sas'}y_{ts'a} \\
% % t = T: & V_{Ts} = \min_a \ell_{Tsa}(y_{Tsa}) \\
% % \end{aligned} \label{kkt condition}
% % \end{equation}

% % Note that \eqref{kkt condition} gives recursive Bellman formulation of the value iteration in dual variable $V_{ts} $. However, since the reward function is dependent on the primal variable, state $y_{tsa} $, it is impossible to completely eliminate the primal variable in the dual constraints. Therefore the problem is not a true MDP but follows the same value iteration methods available to MDPs. 


% % At Nash equilibrium which is also the optimal point of \ref{mdp game}, assume strong convexity holds, the arguments $y_{tsa}^* $, $V_{tsa}^* $ and $\mu_{tsa}^* $ give the minimum value of the optimization problem 
% % \begin{equation}
% % \begin{aligned}
% % \text{primal} \quad&\sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \sum\limits_{a\in\mathcal{A}} \int_0^{y^*_{tsa}}\ell_{tsa}(x)dx = \\
% % \text{dual} \quad&\sum_{tsa} \Big( \int_0^{y^*_{tsa}} \ell_{tsa}(u)\partial u  - \ell_{tsa}(y^*_{tsa})y^*_{tsa}\Big)\\
% % & + \sum_s p_{0s} V_{0s}\\
% % \end{aligned}
% % \end{equation}
% % The optimal values can also be found through Bellman recursion with state dependent rewards. However in order to solve this algorithm, the state action distribution $y_{tsa} $ must be feasible and known a priori. 



% \subsection{Constrained Primal Problem}
% Suppose now we add additional state constraints to \eqref{mdp game}: 
% \[y_{t\bar{s}\bar{a}} \geq d_{t\bar{s}\bar{a}} \quad \forall \bar{s} \in \bar{\mc{S}},\, \bar{a} \in \bar{\mc{A}}, \, t \in [\mc{T}] \]
% % The optimization problem becomes: 
% % \begin{equation}
% % \begin{aligned}
% % \underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \sum\limits_{a\in\mathcal{A}} \int_0^{y_{tsa}}\ell_{tsa}(x)dx\\
% % \mbox{s.t.} &\sum\limits_{a\in\mathcal{A}} y_{t+1, sa} = \sum\limits_{s'\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}P_{sas'}y_{ts'a}, \quad t\in[T-1],\\
% % &\sum\limits_{a\in\mathcal{A}}y_{0sa}=p_s,\\
% % &y_{tsa}\geq 0,\quad \forall s\in\mathcal{S}, a\in\mathcal{A}, t\in[T] \\
% % &y_{t\bar{s}\bar{a}} \geq d_{t\bar{s}\bar{a}} \quad \forall \bar{s} \in \bar{\mc{S}},\, \bar{a} \in \bar{\mc{A}}, \, t \in [\mc{T}]
% % \end{aligned}\label{cmdp game}
% % \end{equation}
% For a set of constraint states $\bar{\mc{S}} $ and constrained actions $\bar{\mc{A}} $. 
% Let $\tau_{t\bar{s}\bar{a}} $ be the dual variable corresponding to this constraint, then lagrangian the constrained \eqref{mdp game} is the following.
% Consider Eqn.\eqref{PMDPCG}, its Lagrangian is:
% \begin{equation}
% \begin{split}
% & L(y_{tsa}, \mu_{tsa}, V_{tsa})  = \sum_{tsa} \Big( \int_0^{y_{tsa}} \ell_{tsa}(u)\partial u - \mu_{tsa}y_{tsa}\Big)\\
% & + \sum\limits_{s\in\mathcal{\bar{S}}, t\in[T]} \tau_{t\bar{s}}\Big(a_{t\bar{s}} - \sum_{a}y_{t\bar{s}a}\Big)_+\\
% & + \sum\limits_{s\in\mathcal{\bar{S}}, t\in[T]} \sigma_{t\bar{s}} \Big( \sum_{a}y_{t\bar{s}a}  -b_{t\bar{s}} \Big)_+ \\
% & + \sum_{t = 1}^T\sum_s \Big(\sum_{as'} P_{ss'a}y_{t-1,sa} - \sum_ay_{tsa}\Big)V_{ts} \\
% & + \sum_s \Big( p_{s} - \sum_ay_{0sa} \Big)V_{0s}\\
% \end{split}
% \end{equation}
% % With the additional complimentarity condition for optimal solution, $(y^c_{tsa}, \mu^c_{tsa}, V^c_{tsa}, \tau^c_{t\bar{s}\bar{a}}) $. 
% % \[\tau^c_{t\bar{s}\bar{a}}(y^c_{t\bar{s}\bar{a}}  - d_{t\bar{s}\bar{a}} ) = 0 \] 
% % This suggests that $\tau^c_{tsa}$ is only non-zero where $y^c_{t\bar{s}\bar{a}}  = d_{t\bar{s}\bar{a}} $, and 
% % $$L(y^c_{tsa}, \mu^c_{tsa}, V^c_{tsa}) = L_c(y^c_{tsa}, \mu^c_{tsa}, V^c_{tsa}, \tau^c_{t\bar{s}\bar{a}}) $$ 

% % Now we wish to find an equivalent, unconstrained version of the constrained problem using the exact penalty theorem \eqref{exactP}. 
% % Then given the non-zero optimal dual variables $\tau^*_{t\bar{s}\bar{a}}$.
% \begin{theorem}
% The optimal strategies and values of Eqn \eqref{CMDPCG} is equivalent to the solution to value iteration algorithm Algorithm \eqref{penalty value iteration} evalulated at $y^c_{tsa}$. Where $\chi_{t\bar{s}\bar{a}}(x) $ is a step function defined by the constraints. 
% \[
% \chi_{tsa}(x) = \begin{cases}
% 1 & x < d_{t\bar{s}\bar{a}} \\
% 0 & x \geq d_{t\bar{s}\bar{a}} \\
% 0 & s \notin \bar{\mc{S}}, a \notin \bar{\mc{A}}\\
% \end{cases}
% \]
% \begin{algorithm}
% \caption{Penalty Value iteration for feasible $y_{tsa}$}
% \begin{algorithmic}[h]
% \Require \(R\), \(P\), \(y_{tsa}\).
% \Ensure \(V^\star\), \(\pi^\star\).
% \ForEach{\(s,\in\mathcal{S}\)}
% \State{\(
% V^\star_{Ts}= \underset{a\in\mathcal{A}}{\mbox{min}} \,\,Q_{Tsa} + k_{Tsa}\chi_{Tsa}(y_{Tsa})\)}
% \State{\(
% \pi^\star_{T}(s)= \underset{a\in\mathcal{A}}{\argmin} \,\,Q_{Tsa} +  k_{Tsa}\chi_{Tsa}(y_{Tsa})\)}
% \EndFor
% \For{\(t=T-1, T-2, \ldots, 0\)}
% \ForEach{\(s\in\mathcal{S}\)}
% \State{\(\displaystyle V^\star_{t}(s)= \underset{a\in\mathcal{A}}{\mbox{min}}\,\, Q_{tsa} +  k_{tsa}\chi_{tsa}(y_{tsa})\)}
% \State{\(\displaystyle \pi^\star_{t}(s) = \underset{a\in\mathcal{A}}{\argmin}\,\, Q_{tsa}+  k_{tsa}\chi_{tsa}(y_{tsa})\)}
% \EndFor
% \EndFor
% \end{algorithmic}
% \label{penalty value iteration}
% \end{algorithm}
% \end{theorem} 
% \begin{proof} TODO Rework this


% From Eqn \eqref{penalty problem}, we already know that the constrained version of the state-dependent potential game, Eqn \eqref{cmdp game}, and the penalized version, Eqn \eqref{pmdp game}, have the same optimal arguments and value when $k_{t\bar{s}\bar{a}} > \tau^c_{t\bar{s}\bar{a}}$ where $\tau^c_{t\bar{s}\bar{a}} > 0 $ are the optimal dual variables from constrained problem, Eqn \eqref{cmdp game}. The function$(\cdot)_+ $ is defined as 
% \[
% \Big(x\Big)_+ = \begin{cases}
% 0  & x \leq 0\\
% x & x > 0\\
% \end{cases}\]
% \begin{equation}
% \begin{aligned}
% \underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \sum\limits_{a\in\mathcal{A}} \int_0^{y_{tsa}}\ell_{tsa}(x)dx \\
% & + \sum\limits_{t\in[T]} \sum\limits_{\bar{s}\in\bar{\mc{S}}} \sum\limits_{\bar{a} \in \bar{\mc{A}}} k_{t\bar{s}\bar{a}} \Big(  d_{t\bar{s}\bar{a}} - y_{t\bar{s}\bar{a}} \Big)_+ \\
% \mbox{s.t.} &\sum\limits_{a\in\mathcal{A}} y_{t+1, sa} = \sum\limits_{s'\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}P_{sas'}y_{ts'a}, \quad t\in[T-1],\\
% &\sum\limits_{a\in\mathcal{A}}y_{0sa}=p_s,\\
% &y_{tsa}\geq 0,\quad \forall s\in\mathcal{S}, a\in\mathcal{A}, t\in[T] \\
% \end{aligned}\label{pmdp game}
% \end{equation}

% It remains to show that the KKT conditions on Eqn \eqref{pmdp game} gives the same solution and arguments as Algorithm \eqref{penalty value iteration}. The KKT conditions on Eqn \eqref{pmdp game} are: 
% \begin{equation}
% \begin{aligned}
% &t = 0: \\
% &\quad  \sum\limits_{a\in\mathcal{A}}y_{0sa}=p_{0s}\\
% &t = 0 \cdots T-1: \\
% &\quad V_{ts} = -\mu_{tsa} + \ell_{tsa}(y_{tsa}) + \\
% & \quad \quad\sum_{s'}P_{s'sa}V_{t+1,s'} +  k_{tsa}\chi_{tsa}(y_{tsa}) \\
% &\quad \sum\limits_{a\in\mathcal{A}} y_{t+1, sa} = \sum\limits_{s'\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}P_{sas'}y_{ts'a} \\
% &t = T: \\
% &\quad V_{Ts} = -\mu_{tsa} +  \ell_{Tsa}(y_{Tsa}) + k_{Tsa}\chi_{Tsa}(y_{Tsa}) \\
% \end{aligned} \label{penalty kkt condition}
% \end{equation}

% From the KKT conditions, Algorithm \eqref{penalty value iteration} can be formulated by noting $\mu_{tsa} \geq 0 $ and $\mu_{tsa} = 0 $ at optimal actions.  Therefore, the optimal solution to Eqn \eqref{pmdp game} can be found by solving with optimal state-action argument to Eqn \eqref{pmdp game}, $y^p_{tsa}$. 

% Once we have solved the constrained problem for the correct penalty values, $\tau^c_{tsa}$, we also concurrently obtain $y^c_{tsa}$, which is equivalent to $ y^p_{tsa} $ when the penalties coefficients satisfy inequality $k_{tsa} > \tau^c_{tsa} $.

% Therefore, the optimal values and strategies of the state-constrained game Eqn \eqref{cmdp game} can be solved through the value iteration method in Algorithm \eqref{penalty value iteration} with $y^c_{tsa} $ 

% \end{proof}

% % For the population $\sum_{as}y_{tsa} $, each individual player is playing a game of 


% % We assume that \eqref{mdp game} with the addition constraints is still feasible and strongly dual. 
% % Using exact penalty theorem, it can be shown that

% % Individual players trying to optimize their value functions through solving the dual of the primal MDP problem. Given the MDP game primal problem, Eqn. \ref{mdp game}, the dual can be written as:  
% % \begin{equation}
% % \begin{aligned}
% % \max_{V_{ts}, y_{tsa}}  & \quad \sum_s V_{0s}p_{0s}  \\
% % \text{s.t } & V_{ts} \leq \sum_{s'} P(s'| s, a)V_{t+1,s'} + \ell_{tsa}(y_{tsa}) \quad \\
% % & \forall \, s \in \mc{S}, a\in \mc{A}, t \in [T-1] \\
% % & V_{Ts} \leq \ell_{tsa}(y_{tsa}) \quad \forall \, s \in \mc{S},\,\, a\in \mc{A}
% % \end{aligned} \label{unconstrained dual}
% % \end{equation}
% % From this we can derive the value iteration method shown for latency functions $\ell_{tsa}(y_{tsa}) $. Let the Q function be defined as following: 
% % \begin{equation}\label{q function}
% % Q_{tsa}(y_{tsa}) = \sum_{s'} P(s'| s, a)V_{t+1,s'} + \ell_{tsa}(y_{tsa}) \\
% % \end{equation}
% % The difference $V^*_{ts} -  Q_{tsa}(y^*_{tsa}) = \mu^*_{tsa} \geq 0$ is the dual variable of constraint $y_{tsa} \geq 0 $, and is also the inefficiency of the action $a$. Any action $\bar{a} $ whose inefficiency is zero is the optimal action at that particular state and time. 


% % Which leads to the value iteration method Alg. \ref{value iteration}. 


% % \begin{theorem}
% % Assuming existing players have reached nash equilibirum, and the rewards are state dependent $R_{tsa}(y_{tsa}) $, algorithm \ref{value iteration} with optimal  $y^*_{tsa} $ is the dynamic programming problem that any new player solves entering the game at time $t $.

% % Furthermore, the best reward that the new player can gain is defined by 
% % \[\min_s V^*_{ts}\]
% % \end{theorem}

% % \begin{proof}
% % Since the algorithm depends on current state-action distribution, $y_{tsa}$. At Nash Equilibrium the constraints would be: 
% % \[V_{ts} \leq \sum_{s'} P(s'| s, a)V_{t+1,s'} + \ell_{tsa}(y^*_{tsa}) \]
% % \[V_{Ts} \leq \ell_{tsa}(y^*_{tsa}) \]
% % Any player entering at time t would need to maximize its value function according to $V_{ts} $. Since the game is non-atomic, the new player would not affect the state depedent reward functions. Therefore, the new player's optimal policy can be found from algorithm \ref{value iteration}.
% %  % optimal policy for each individual player will be different in the finite horizon case.  
% % \end{proof}



% % Suppose we impose constraint $y_{t\bar{s}\bar{a}} \leq d_{t\bar{s}\bar{a}} $ for one state $\bar{s} $ and all times t, and suppose it was violated during time step $\bar{t}$. From an individual game player's perspective, the exact penalty function coefficients $k_t(\bar{s},\bar{a}) $,  directly offsets the value functions at constrained optimal $y_c^*(s,a)$.  

% % Using the exact penalty theorem, we find the minimum coefficient $k_{\bar{t}\bar{s}\bar{a}} \geq \tau^*_{\bar{t}\bar{s}\bar{a}} $ to ensure that the optimal solutions are between the penalized problem and the unconstrained problem are the same. However in order to ensure that the next player will also avoid the constraints, additional "toll" need to be charged. 


% % \begin{theorem}
% % In addition to $\tau^*_{\bar{t}\bar{s}}$ the dual variable's optimal value corresponding to the constraint $y_{t\bar{s}\bar{a}} \leq d_{t\bar{s}} $ in problem \eqref{MDP game}. Let 
% % \[k_{\bar{t}\bar{s}\bar{a}} > \max\{\tau^*_{\bar{t}\bar{s}\bar{a}}, \mu_{\bar{t}\bar{s}a_{new}}   \}\]
% % \[a_{new} = \text{argmin}_{a \neq \bar{a}} Q_{\bar{t}\bar{s}a} \]
% % Then we can guarantee that the next player will not choose to violate the constraint $y_{\bar{t}\bar{s}\bar{a}} \leq d_{\bar{t}\bar{s}\bar{a}} $

% % \end{theorem}

% % \begin{proof}
% % From the exact penalty theorem, the solution to the unconstrained problem \eqref{MDP Game} and the constrained problem \eqref{cMDP game} share the same value and argument. 
% % \begin{equation}
% % \begin{aligned}
% % \underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \sum\limits_{a\in\mathcal{A}} \int_0^{y_{tsa}}\ell_{tsa}(x)dx\\
% % \mbox{s.t.} &\sum\limits_{a\in\mathcal{A}} y_{t+1, sa} = \sum\limits_{s'\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}P_{s'as}y_{ts'a}, \quad t\in[T-1],\\
% % &\sum\limits_{a\in\mathcal{A}}y_{0sa}=p_s,\\
% % & y_{t\bar{s}\bar{a}} \leq d_{t\bar{s}\bar{a}}, \\
% % &y_{tsa}\geq 0,\quad \forall s\in\mathcal{S}, a\in\mathcal{A}, t\in[T]
% % \end{aligned}\label{cMDP game}
% % \end{equation}

% % For at the optimal solution of this constrained MDP game, the dual value iteration method occurs according to algorithm \ref{constrained value iteration}. Here we see the value of $k_{t\bar{s}\bar{a}} $ directly offsets the Q-functions at the times when the unconstrained solution violated the state constraints.



% % Suppose the violated constraint occurs at $\bar{t}, \bar{s}, \bar{a} $. Let $\tilde{\mu} $ be the smallest inefficiency of the set of actions available at $\bar{s} $, excluding optimal action $\bar{a} $. If $k_{\bar{t}\bar{s}\bar{a}} > \tilde{\mu} $, then $\bar{a} $ is no longer the optimal, and so the player will not choose $\bar{a} $ as optimal policy. Therefore, the original constraint $y_{t\bar{s}\bar{a}} \leq d_{t\bar{s}\bar{a}} $ cannot be violated at $\bar{t} $ if the original solution was feasible. 

% % Since $k_{\bar{t}\bar{s}\bar{a}} > \tau^*_{\bar{t}\bar{s}\bar{a}} $, then we still satisfy the exact penalty theorem, and so the optimal solution and arguments of the penalized problem still correspond to the constrained problem's solution and arguments. 
% % \end{proof}

% % \begin{theorem}
% % For a new player entering the game at time $t $, their best expected reward is upperbounded by the optimal value function at time $t $. 
% % \[\max_{s} \tilde{V}_{ts} \]
% % Where $\tilde{V}_{ts} $ is the result of solving algorithm \ref{constrained value iteration}. Furthermore, the player can achieve this value by starting at state $s = \text{argmax} V_{ts} $ and follow optimal policy $\pi_{ts}^* $from algorithm \ref{constrained value iteration}.
% % \end{theorem}
% % \begin{proof}
% % This follows from the fact that the value functions is equivalent to the expected sum of rewards over time.
% % \end{proof}
% % \begin{proof}
% % 
% % Note that the KKT conditions of the primal optimization problem with the exact penalty terms gives the same value iterations as the not penalized, unconstrained problem when the constraints are not active. But gives the following inequalities when the constraints are active. 
% % \[ \tilde{V}_t(s) \leq \sum_{s'} P(s'| s, a)\tilde{V}_{t+1}(s') + R_t(s,a) + k_t(s,a) \quad \forall \, s \in \mc{S}, a\in \mc{A}, t \in [T-1] \]
% % \[ \tilde{V}_T(s) \leq R_T(s,a)+ k_T(s,a) \quad \forall \, s \in \mc{S},\,\, a\in \mc{A} \]

% % Then since $k_t(s,a) > \tau_t^*(s,a) $, we note that where $\tau_t^*(s,a) = 0 $, we can remove the constraint and equivalently set $k_t(s,a) = 0 $. Therefore, the previous KKT conditions hold both when constraints are active and not active. Finally they lead to the value iteration method outlined in Algorithm \ref{constrained value iteration}.

% % Finally for any additional player with a choice of starting position, their optimal choice to minimize $\tilde{V}_0$ would be to choose the state with the smallest initial value function. 
% % \end{proof}

% % \begin{theorem}
% % Assume there exists a feasible, non-zero toll, $\tau^* $ corresponding to constraint  $y_t(s,a) \leq d_t(s,a)$ for Eqn. \ref{MDP}. Then for $V_0^*(s)$ the optimal solution of the dual problem,
% % % For the following MDP problem, with the added constraint  $y_t(s,a) \leq d_t(s) $. 
% % % \begin{equation}\label{MDP}
% % % \begin{aligned}
% % % \text{maximize}\quad &\sum_{t\in\mathcal{T}} \sum_{s\in\mathcal{S}} \sum_{a\in\mathcal{A}} \int_0^{y_t(s,a)} c_t(s,a) \partial y_t(s,a) \\
% % % \text{s.t.} \,\,& \sum\limits_{a\in\mathcal{A}} y_{t+1}(s', a) = \sum\limits_{s\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}\Gamma(s'\mid s, a)y_t(s, a),\\
% % % &\sum\limits_{a\in\mathcal{A}}y_0(s, a)=p_0(s),\\
% % % &y_t(s, a)\geq 0,\\
% % % \end{aligned}
% % % \end{equation}
% % then any additional agents added to network will avoid the constrained state. 
% % \end{theorem}
% % \begin{proof}
% % Consider an optimal solution to the unconstrained problem, Eqn. \ref{MDP}, $y^*_t(s,a)$, for some convex reward function $R_t(s,a)$. 
% % \begin{equation}
% % \begin{aligned}
% % \underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \sum\limits_{a\in\mathcal{A}} R_t(s,a)\\
% % \mbox{s.t.} &\sum\limits_{a\in\mathcal{A}} y_{t+1}(s,a) = \sum\limits_{s'\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}P(s'|s,a)y_{t+1}(s,a), \quad t\in[T-1],\\
% % &\sum\limits_{a\in\mathcal{A}}y_0(s,a)=p(s),\\
% % &y_t(s,a)\geq 0,\quad \forall s\in\mathcal{S}, a\in\mathcal{A}, t\in[T]
% % \end{aligned}\label{MDP}
% % \end{equation}
% % Suppose constraints $y_t(\bar{s},\bar{a}) \leq d_t$ are added for all t. Let $x_t^*(s,a)$ be the solution to Eqn.\ref{cMDP}. 
% % \begin{equation}
% % \begin{aligned}
% % \underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \sum\limits_{a\in\mathcal{A}} R_t(s,a)\\
% % \mbox{s.t.} &\sum\limits_{a\in\mathcal{A}} y_{t+1}(s,a) = \sum\limits_{s'\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}P(s'|s,a)y_{t+1}(s,a), \quad t\in[T-1],\\
% % &\sum\limits_{a\in\mathcal{A}}y_0(s,a)=p(s),\\
% % &y_t(s,a)\geq 0,\quad \forall s\in\mathcal{S}, a\in\mathcal{A}, t\in[T] \\
% % &y_t(\bar{s},\bar{a}) \leq d_t, \quad \forall  t\in[T]
% % \end{aligned}\label{cMDP}
% % \end{equation}
% % Finally consider the exact penalty from Eqn. \ref{cMDP}, in the form : $\sum_{t\in[T]} k_t(y_t(\bar{s},\bar{a}) - d_t)_+ $, where $k_t > \tau^*_t $, the optimal dual variables, and the optimal solution of the unconstrained problem, Eqn.\ref{exMDP}, with the exact penalty term, $z^*_t(s,a) $. 
% % \begin{equation}
% % \begin{aligned}
% % \underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \sum\limits_{a\in\mathcal{A}} R_t(s,a) + \sum_{t\in[T]} k_t(y_t(\bar{s},\bar{a}) - d_t)_+\\
% % \mbox{s.t.} &\sum\limits_{a\in\mathcal{A}} y_{t+1}(s,a) = \sum\limits_{s'\in\mathcal{S}}\sum\limits_{a\in\mathcal{A}}P(s'|s,a)y_{t+1}(s,a), \quad t\in[T-1],\\
% % &\sum\limits_{a\in\mathcal{A}}y_0(s,a)=p(s),\\
% % &y_t(s,a)\geq 0,\quad \forall s\in\mathcal{S}, a\in\mathcal{A}, t\in[T] \\
% % \end{aligned}\label{exMDP}
% % \end{equation}

% % If $y^*_t(\bar{s},\bar{a}) < d_t $, then adding additional population $\partial y $ will not violate the constraints either. Therefore we only consider the case when the constraint is active. Ie. $y^*_t(\bar{s},\bar{a}) \geq d_t $.


% % The gradient of the Lagrangian with respect to $y_t(s,a) $ gives rise to value iteration. For each $t = 0\cdots, T-1 $, the gradient of the constrained Lagrangian of Eqn.\ref{cMDP} with respect to $y_t(\bar{s}, \bar{a}) $ is the following.

% % \[ \nabla R_t(\bar{s}, \bar{a})  + \sum_{s'} P(s'| \bar{s}, \bar{a})  + \mu_t(\bar{s}, \bar{a}) - V_t(\bar{s}) + \tau_t \]

% % For optimal $x_t^*(\bar{s},\bar{a}), V^*_t(\bar{s}), V^*_{t+1}(\bar{s}), \mu^*_t(\bar{s}, \bar{a}) $, $\frac{\partial L_c}{y_t(\bar{s}, \bar{a})} = 0 $. Since we assumed that the constraint is active, $ x_t^*(\bar{s},\bar{a})  = d_t > 0 $. From complimentary slackness, $\mu^*_t(\bar{s},\bar{a}) = 0 $. 

% % \[ \nabla R_t(\bar{s}, \bar{a})  + \sum_{s'} P(s'| \bar{s}, \bar{a})V_{t+1}(s') - V_t(\bar{s}) + \tau_t = 0\]

% % Similarly for a different action $a_2 $,  the following is true at optimal values, $x_t^*(\bar{s},a_2), V^*_t(\bar{s}), V^*_{t+1}(\bar{s}), \mu^*_t(\bar{s}, a_2) $, $\frac{\partial L_c}{y_t(\bar{s}, a_2)} = 0  $

% % \[ \nabla R_t(\bar{s}, a_2)  + \sum_{s'} P(s'| \bar{s}, a_2)V_{t+1}(s')  + \mu_t(\bar{s}, a_2) - V_t(\bar{s}) = 0\]

% % The two KKT conditions have $V_t(\bar{s}) $ and $V_{t+1}(s') \quad \forall s' \in \mathcal{S}$ in common, solving for $\tau_t $:
% % \begin{equation}
% % \begin{split}
% % \tau_t & = \nabla R_t(\bar{s}, a_2) - \nabla R_t(\bar{s}, \bar{a}) \\
% % & + \sum_{s'} P(s'| \bar{s}, a_2)V_{t+1}(s')  - \sum_{s'} P(s'| \bar{s}, \bar{a})V_{t+1}(s') \\
% % & + \mu_t(\bar{s}, a_2) \\
% % \end{split}
% % \end{equation}

% % From exact penalty theorem, Eqn.\ref{exMDP} must have the same solution arguments as Eqn.\ref{cMDP}. Let $W_t(\bar{s}) $ be the value functions for the dual of Eqn.\ref{exMDP}. The following relationship must hold: 
% % \begin{equation}
% % \begin{aligned}
% % \nabla R_t(\bar{s}, \bar{a})  + \sum_{s'} P(s'| \bar{s}, \bar{a})W_{t+1}(s')) - V_t(\bar{s})  &= \\
% % \nabla R_t(\bar{s}, a_2)  + \sum_{s'} P(s'| \bar{s}, \bar{a})W_{t+1}(s')) - V_t(\bar{s})  &
% % \end{aligned}
% % \end{equation}


==> problemFormulation.tex <==
% \section{Problem Formulation}\label{problemFormulation}

\section{Problem Formulation}\label{problemFormulation}
Consider a finite horizon, Markov Decision Process (MDP) congestion game, where a group of players individually solves an MDP to maximize expected self gain while competing for global resources. We assume that all players have the same set of possible actions and stochastic transitions. This type of finite horizon, Markov Decision Process congestion game (MDPCG) is formulated as a convex optimization problem in \cite{MDPCongestionGame}. 
% * <yueyu@uw.edu> 2018-08-27T17:45:45.274Z:
% 
% Emphasize the role of MDP in this setup, such as "each player solves an MDP"
% Reference to later section is bizarre in this place. Consider replace with "A finite horizon MDPCG ... a convex optimization \cite{Dan's paper}".
% Does "finite resources" refer to capacity constraints? -If so, then better focus the paragraph on the unconstrained MDPCG, and emphasize the constraints later, given it is the main contribution of the paper. 
% 
% ^ <crab.apples00@gmail.com> 2018-08-30T04:15:23.491Z:
% 
% Resources refer to the congestion effects, ie the more people crowd a state, the less gain everybody gets. I've changed it to global resources hopefully that makes it clearer
%
% ^.

In this paper, we develop a dual interpretation for the role that state constraints play in MDPCG: through a social planner's perspective and individual players' perspective. Players will attempt to maximize their individual objectives by finding an optimal sequence of actions, while a social planner strives for game-level objectives, such as maximizing total gain or enforcing state constraints. To achieve these objectives, the planner cannot impose explicit constraints, but instead can adjust individual objectives to incentivize/discourage certain actions. A toll/reward method is developed for implicitly realizing global state dependent constraints .
% * <yueyu@uw.edu> 2018-08-27T17:59:54.011Z:
% 
% Constraints should be emphasized more: we aim to  introduce capacity constraints in MDPCG. Using duality theory, such modification can be interpreted from both an individual player and a social planner perspective.  
%  
% "alternative objective" is not very informative. Consider "global/social objective" instead; it echos better to the "individual objective" of each player. 
% 
% ^.

The rest of the paper is organized as follows: in Section \ref{notation}, we introduce the convex optimization model of state-constrained MDPCG. Section \ref{convergence} connects the constrained optimal solution to Wardrop equilibrium with respect to a generalized cost function. In Section \ref{dualFormulation}, we perform simulations of repeated game play using a fixed step-sized Frank Wolfe Method. The simulations show that when the cost functions are adjusted for tolls, players indeed converge at the optimal strategy that does not violate corresponding state constraints.

% * <yueyu@uw.edu> 2018-08-27T20:19:22.244Z:
% 
% When possible, active voice is preferred than a passive one.
% 
% ^.

==> rewardUncertainty.tex <==
\section{Reward Uncertainty}
Here we introduce slightly different notation: 
\[y_{ts} = \begin{pmatrix}
y_{tsa_1} \\ y_{tsa_2}\\\vdots\\y_{tsa_m}\\
\end{pmatrix} \in \reals^{|\mc{A}|} \]
\[
\ell_{ts}(y_{ts}) = \begin{pmatrix}
\ell_{tsa_1}(y_{tsa_1}) \\ \ell_{tsa_2}(y_{tsa_2})\\\vdots\\\ell_{tsa_m}(y_{tsa_m})\\
\end{pmatrix} \in \reals^{|\mc{A}|}
\]
The optimization problem can be rewritten in the new vector variable form: 
\begin{equation}
\begin{aligned}
\underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \int_0^{y_{ts}}\ell_{ts}(x)dx\\
\mbox{s.t.} & \ones^T y_{t+1, s} = \sum\limits_{s'\in\mathcal{S}}P_{s\cdot s'}^Ty_{ts'}, \quad t\in[T-1],\\
&\ones^Ty_{0s}=p_s,\\
&y_{ts}\geq 0,\quad \forall s\in\mathcal{S}, t\in[T]
\end{aligned}\label{mdp game vector}
\end{equation}

\subsection{Uncertainty Model}
For each individual solving the problem, their model of the reward may be entirely experience based and therefore prone to uncertainty. 

Here, we model their uncertainty as the following: for $(t,s,a)$, the reward can be anywhere within the following ellipse, which is also state dependent in its mean value
\begin{equation}
\begin{aligned}
\ell_{ts}(x) &\in \mathcal{E}_{ts} \quad \forall \,\, x \in [0,1] \\
& \in \{R_{ts}x + Q_{ts}u_{ts}\, | \quad \norm{u}_2 \leq 1\} \\
\end{aligned}
\end{equation}
Where $R_{ts} \in \reals^{|S| \times |S| } $ is a time and state dependent matrix. 

Suppose we are considering worstcase scenario, the objective can be rewritten as: 
\begin{equation}
\begin{aligned}
&\sup\{\ones^T\sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}} \int_0^{y_{ts}}\ell_{ts}(x)dx\} \\
= &\sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}}  \ones^T\int_0^{y_{ts}}R_{ts}xdx + \sup\{\ones^T\int_0^{y_{ts}}Q_{ts}u dx | \norm{u}_2 \leq 1\} \\
\leq &\sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}}\half\norm{R_{ts}{y_{ts}}}^2_2 + \sup\{\norm{u_{ts}^TQ_{ts}^Ty_{ts}}_2| \norm{u}_2 \leq 1\} \\
\leq &\sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}}\half\norm{R_{ts}{y_{ts}}}^2_2 +\norm{Q_{ts}^Ty_{ts}}_2 \\
\end{aligned}
\end{equation} 
Then the optimization problem becomes: 
\begin{equation}
\begin{aligned}
\underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}}\half\norm{R_{ts}{y_{ts}}}^2_2 +\norm{Q_{ts}^Ty_{ts}}_2 \\
\mbox{s.t.} & \ones^T y_{t+1, s} = \sum\limits_{s'\in\mathcal{S}}P_{s\cdot s'}^Ty_{ts'}, \quad t\in[T-1],\\
&\ones^Ty_{0s}=p_s,\\
&y_{ts}\geq 0,\quad \forall s\in\mathcal{S}, t\in[T]
\end{aligned}\label{mdp game vector}
\end{equation}

The Lagangian becomes
\begin{equation}
\begin{aligned}
L(y_{ts}, V_{ts}, \mu_{ts}) & = \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}}\half\norm{R_{ts}y_{ts}}^2_2 +\norm{Q_{ts}^Ty_{ts}}_2 \\
& + \sum\limits_{t \in [1,T]}\sum\limits_{s\in\mc{S}} V_{ts}\Big(\sum\limits_{s' \in \mc{S}}P^T_{s\cdot s'} y_{t-1,s'} - \ones^Ty_{ts}\Big) \\
& + \sum\limits_{s \in \mc{S}}V_{0s}\Big(p_s - \ones^Ty_{0s}\Big) \\
& - \sum\limits_{s \in \mc{S}}\sum\limits_{t \in[T]}\mu_{ts}^Ty_{ts} \\
\end{aligned}
\end{equation}

Then the corresponding KKT conditions for the value iteration is: 

\begin{equation}
\begin{aligned}
&t = 0 \cdots T-1: \\
&\quad V_{ts}\ones = -\mu_{ts} + R_{ts}y_{ts} + \frac{1}{\norm{Q_{ts}^Ty_{ts}}_2}Q_{ts}Q_{ts}^Ty_{ts}\\
& \quad\quad + \sum_{s'}P_{s'\cdot s}V_{t+1,s'} \\
&t = T: \\
&\quad V_{Ts}\ones = -\mu_{tsa}  + R_{Ts}y_{Ts} + \frac{1}{\norm{Q_{Ts}^Ty_{Ts}}_2}Q_{Ts}Q_{Ts}^Ty_{Ts}\\
\end{aligned} \label{robust kkt condition}
\end{equation} 

We can estimate the worst case of $\frac{1}{\norm{Q_{ts}^Ty_{ts}}_2}Q_{ts}Q_{ts}^Ty_{ts} $ by the following inequality based on Cauchy-Schwarz inequality: 
\[\frac{1}{\norm{Q_{ts}^Ty_{ts}}_2}Q_{ts}Q_{ts}^Ty_{ts} \geq -\norm{Q_{ts}}_2 \]

Then the worst case dual problem is the following: 
\begin{equation}
\begin{aligned}
\underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}}\half\norm{R_{ts}{y_{ts}}}^2_2  - y^T_{ts}R_{ts}y_{ts}+ \sum\limits_{s \in \mc{S}}p_sV_{0s} \\
\mbox{s.t.} & V_{ts}\ones \leq R_{ts}y_{ts} - \norm{Q_{ts}}_2  + \sum_{s'}P_{s'\cdot s}V_{t+1,s'} \\
&V_{Ts}\ones \leq R_{Ts}y_{Ts} - \norm{Q_{Ts}}_2 \\
\end{aligned}\label{mdp game vector}
\end{equation}
Notice that since $\norm{Q_{ts}}_2  = \lambda_{max} $, this is equivalent to offsetting the reward function by the worst possible variation, to obtain a robust reward function $R_{ts} - \lambda_{max}(Q_{ts}) $
% \begin{equation}
% \begin{aligned}
% \underset{y}{\mbox{min.}} & \sum\limits_{t\in[T]}\sum\limits_{s\in\mathcal{S}}2\norm{R_{ts}{y_{ts}}}^2_2 +\norm{Q_{ts}^Ty_{ts}}_2 \\
% \mbox{s.t.} & \ones^T y_{t+1, s} = \sum\limits_{s'\in\mathcal{S}}P_{s\cdot s'}^Ty_{ts'}, \quad t\in[T-1],\\
% &\ones^Ty_{0s}=p_s,\\
% &y_{ts}\geq 0,\quad \forall s\in\mathcal{S}, t\in[T]
% \end{aligned}\label{mdp game vector}
% \end{equation}
